A Survey on LLM Test-Time Compute via Search: Tasks, LLM Profiling, Search Algorithms, and Relevant Frameworks

LLM test-time compute (or LLM inference) via search has emerged as a promising research area with rapid developments. However, current frameworks often adopt distinct perspectives on three key aspects: task definition, LLM profiling, and search procedures, making direct comparisons challenging. Moreover, the search algorithms employed often diverge from standard implementations, and their specific characteristics are not thoroughly specified. This survey aims to provide a comprehensive but integrated technical review on existing LIS frameworks. Specifically, we unify task definitions under Markov Decision Process (MDP) and provides modular definitions of LLM profiling and search procedures. The definitions enable precise comparisons of various LLM inference frameworks while highlighting their departures from conventional search algorithms. We also discuss the applicability, performance, and efficiency of these methods. For ongoing paper updates, please refer to our GitHub repository: https://github.com/xinzhel/LLM-Search.

==> sections/change.tex <==
\section{Version Changes}
For readers who viewed the preprint on 17 Jan 2025 on arXiv, below are the significant updates you may want to pay attention to.
% \begin{markdown}
\begin{itemize}
    \item (Modify Figure 1) Remove references to Sections 2, 3, and 4 to avoid duplication.
    \item (Add in Section 2) Insert new paragraph "Conceptual Foundations of MDPs" and add discussion on embodied tasks and combinatorial tasks.
    \item (Add in Table 2) Include common benchmarks.
    \item (Add in Section 3) Introduce a stochastic policy and several new evaluators.
    \item (Add in Section 5) Add two new papers on LLM inference via MCTS, decoupled from frameworks that include LMPR training.
    \item (Modify Sections) Reorder the "Related Work" section (currently Section 7) to appear before the "Discussion" section (currently Section 8), so that related work is introduced earlier to be mentioned in the "Discussion".
    \item (Add in Sections 5, 6, 7) Incorporate 11 new ICLR2025 papers.
    \item (Add in Section 7) Specify fine-tuning frameworks for test-time computation (e.g., ReST).
    \item (Add in Section 8) Include extra perspectives and future work.
    \item (Remove in Section 8) Delete the duplicate "Beyond Finite, Fixed Search Space" paragraph.
\end{itemize}
% \end{markdown}

% <!-- * Change the section title "LLM inference + Search Beyond Sequential Decision Making" to "LLM inference + Search Beyond Task Decomposition" -->
% <!-- how the framework TS-LLM fits in the RLHF scenarios -->

==> sections/format.tex <==
\section{Submission of papers to TMLR}

TMLR requires electronic submissions, processed by
\url{https://openreview.net/}. See TMLR's website for more instructions.

If your paper is ultimately accepted, use option {\tt accepted} with the {\tt tmlr} 
package to adjust the format to the camera ready requirements, as follows:
\begin{center}  
  {\tt {\textbackslash}usepackage[accepted]\{tmlr\}}. 
\end{center}
You also need to specify the month and year
by defining variables {\tt month} and {\tt year}, which respectively
should be a 2-digit and 4-digit number. To de-anonymize and remove mentions
to TMLR (for example for posting to preprint servers), use the preprint option,
as in {\tt {\textbackslash}usepackage[preprint]\{tmlr\}}. 

Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to TMLR must be prepared according to the
instructions presented here.

Authors are required to use the TMLR \LaTeX{} style files obtainable at the
TMLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for TMLR and other journal information are available online on
the TMLR website.
The file \verb+tmlr.pdf+ contains these
instructions and illustrates the
various formatting requirements your TMLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+tmlr.sty+ and \verb+tmlr.bst+ (to be used with \LaTeX{}2e). The file
\verb+tmlr.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 6.5~inches wide and
9~inches long. The left margin is 1~inch.
Use 10~point type with a vertical spacing of 11~points. Computer Modern Bright is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in bold and left-aligned.
All pages should start at 1~inch from the top of the page.

Authors' names are
set in boldface. Each name is placed above its corresponding
address and has its corresponding email contact on the same line, in italic 
and right aligned. The lead author's name is to be listed first, and
the co-authors' names are set to follow vertically.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

First level headings are in bold,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in bold,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in bold,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis, using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textbf{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches.\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}. Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Broader Impact Statement}
In this optional section, TMLR encourages authors to discuss possible repercussions of their work,
notably any potential negative impact that a user of this research should be aware of. 
Authors should consult the TMLR Ethics Guidelines available on the TMLR website
for guidance on how to approach this subject.

\subsubsection*{Author Contributions}
If you'd like to, you may include a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors. Only add
this information once your submission is accepted and deanonymized. 

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.
Only add this information once your submission is accepted and deanonymized. 


==> tables/mcts.tex <==
\begin{algorithm*}
\caption{MCTS for LLM-based Planning. Details are ignored for the following procedures: one at a pass or all at a pass for \textsc{Sample\_Actions} } 
\label{alg:llm_mcts}
\small
\textbf{Input}: Initial state $s_1$, Number of roll-outs $K$, Depth limit $L$, action sampling size $N$, LLM-Profiled Roles: $\text{glm}_\text{actor}$, 
$\text{Simulator}$ (e.g., $\text{glm}_\text{transition}$), $\text{glm}_\text{eval}$ \\
\textbf{Output}: action $a$

% Begin two-column layout inside full-width algorithm
\noindent
\begin{minipage}[t]{0.48\textwidth}
    \begin{algorithmic}[1]
        \For{$k \in \{0, \ldots, K-1 \}$}
        \For{$t \in \{0, \ldots, L-1 \}$}
            \If{$s_t$ not terminal}
                \State $\mathbf{a}_t^{(0\ldots N)}$ $\gets$ \Call{Sample\_Actions}{$s_t, N$}                  
                \State $\mathbf{s}_{t+1}^{(0\ldots N)}$ $\gets$ \Call{Simulate}{$a_t, s_t$} 

                \State Add $\mathbf{s}_{t+1}^{(0\ldots N)}$ to children
                
                \State $V_t^{(0\ldots N)} \gets$ \Call{Evaluate}{$\mathbf{a}_t$}
            \EndIf
        \EndFor
        \EndFor
        \State \textbf{return} $a$

        \Procedure{Evaluate}{$\mathbf{s}_t$, $\mathbf{a}_t$} 
        % State-action value function
        \State $\mathbf{a}_t \sim \text{glm}_\text{actor} \left(\mathbf{a} \mid s_t \right)$
        \State \textbf{return} $\mathbf{a}_t$
        \EndProcedure
    \end{algorithmic}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.48\textwidth}
    \begin{algorithmic}[1]
    \Procedure{Search}{$h, b, \mathcal{T}, N$}
            \State $n \gets 0$
            \While{$n < N$}
                \State $s \sim b(s)$
                \State \textsc{Simulate}($s, h, \text{False}, 0, \mathcal{T}$)
                \State $n \gets n + 1$
            \EndWhile
            \State \textbf{return} $\arg \max_{a \in A} Q(h, a)$
        \EndProcedure
        \Procedure{Rollout}{$s, h, \text{done}, d$}
            \If{$\gamma^d < \epsilon$ or $\text{done} = \text{True}$}
                \State \textbf{return} 0
            \EndIf
            \State $a \sim \pi_\text{rollout}(h, \cdot)$
            \State $(s', o, r, \text{done}) \sim \mathcal{G}(s, a)$
            \State $h' \gets \textsc{PushBack}(h, [a^*, o]), d' \gets d + 1$
            \State \textbf{return} $r + \gamma \cdot \textsc{Rollout}(s', h', \text{done}, d')$
        \EndProcedure
    \end{algorithmic}
\end{minipage}
% End of two-column layout inside full-width algorithm
\end{algorithm*}

==> tables/planning-comparison.tex <==
\begin{table*}[ht!]
    \centering
    \begin{tabular}{p{3.5cm}p{1.25cm}p{1.25cm}p{1.5cm}p{1.5cm}p{1.5cm}p{2cm}p{2cm}p{2cm}}
    \toprule
                    & Planning?
                    & Step(s) (1/1+) % AR Step for A Plan 
                    & Path(s) (1/1+) % Not Complete Plans
                    & Lookahead 
                    & Backtrack 
                    & Closed-loop?
                    % & Related Work
                    
    \\ \midrule
     \textbf{Search-Based}
     \\ \addlinespace
     ToT-BFS \citep{yao2023tree}
     & Always
     & 1+ & 1+
     & \xmark & \xmark 
     & \xmark
     \\ \addlinespace

    ToT-DFS \citep{yao2023tree}
     & Always
     & 1+ & 1+
     & \cmark & \cmark 
     & \xmark
     \\ \addlinespace
     
     RAP \citep{hao-etal-2023-reasoning}
     & Always
     & 1+ & 1+
     & \cmark & \xmark 
     & \xmark
     \\ \addlinespace

     LLM-MCTS \citep{zhao2023large}
     & Always
     & 1+ & 1+
     & \cmark & \xmark 
     & \xmark
     \\ \addlinespace

     LATS \citep{zhou2024language}
     & Always
     & 1+ & 1+
     & \cmark & \xmark 
     & \cmark
     \\ \addlinespace

     % GDP-Zero \citep{yu2023promptbased}
     % \\ \addlinespace

     % PG-TD \citep{zhang2023planning}
     % \\ \addlinespace


     LLM-Best \citet{koh2024tree}
     & Always
     & 1+ & 1+
     & \cmark & \cmark 
     & 
     \\ \addlinespace

    \textbf{Re-ranking}
     \\ \addlinespace
     
     Self-Consistency \citep{wang2023selfconsistency}
     & Always Not
     & 1 & 1+ 
     & \xmark & \xmark
     & \xmark
     \\ \addlinespace
     
     \textbf{Reasoning-only}
     \\ \addlinespace

     CoT \citep{wei2022chain} 
     & Always Not
     & 1 & 1
     & \xmark & \xmark
     & \xmark
     \\ \addlinespace

    \textbf{Reasoning-then-acting}
     \\ \addlinespace
     ReAct \citep{yao2023react} 
     & Maybe
     & 1+ & 1
     & \cmark & \xmark
     & \cmark
     \\ \addlinespace

    \textbf{Task Decomposition}
    \\ \addlinespace
    
     Least to Most \citep{zhou2023leasttomost}
     & NA
     & 1+ & 1
     & \xmark & \xmark
     & \xmark
     \\ \addlinespace
     
     HuggingfaceGPT \citep{shen2023hugginggpt}
     & NA
     & 1+ & 1
     & \xmark & \xmark
     & \xmark
     
     \\ \bottomrule
    \end{tabular}
    \caption{Comparisons of Search-Based Planning with Other Prompting (or Agentic) Frameworks for Planning}
    \label{tab:comparison}
\end{table*}






